Accurately Estimating Unreported Infections using Information Theory

One of the most significant challenges in combating against the spread of infectious diseases was the difficulty in estimating the true magnitude of infections. Unreported infections could drive up disease spread, making it very hard to accurately estimate the infectivity of the pathogen, therewith hampering our ability to react effectively. Despite the use of surveillance-based methods such as serological studies, identifying the true magnitude is still challenging. This paper proposes an information theoretic approach for accurately estimating the number of total infections. Our approach is built on top of Ordinary Differential Equations (ODE) based models, which are commonly used in epidemiology and for estimating such infections. We show how we can help such models to better compute the number of total infections and identify the parametrization by which we need the fewest bits to describe the observed dynamics of reported infections. Our experiments on COVID-19 spread show that our approach leads to not only substantially better estimates of the number of total infections but also better forecasts of infections than standard model calibration based methods. We additionally show how our learned parametrization helps in modeling more accurate what-if scenarios with non-pharmaceutical interventions. Our approach provides a general method for improving epidemic modeling which is applicable broadly.

==> Sections/data.tex <==
\subsection*{Datasets}
We use the following publicly available datasets for our study:

\begin{enumerate}
    \item \textbf{New York Times reported infections~\cite{nytimeswebsite}:}
    This dataset ($\textsc{NYT-R}\mathrm{inf}$) consists of the daily time sequence of reported COVID-19 infections $D_{\mathrm{reported}}$ and the mortality $D_{\mathrm{mortality}}$ (cumulative values) for each county in the US starting from January 21, 2020 to current.
    
    \item \textbf{Serological studies~\cite{havers2020seroprevalence,CDCTracker}:} This dataset consists of the point and 95\% confidence interval estimates of the prevalence of antibodies to SARS-CoV-2 in 10 US locations every 3–4 weeks from March to July 2020. For each location, CDC works with commercial laboratories to collect the blood specimens in the population and test them for antibodies to SARS-CoV-2. Each specimen collection period ranges from 6 to 14 days. As suggested by prior work~\cite{jones2021estimated,peluso2021sars}, these serological studies have high sensitivity to antibodies for 6 months after infections. Hence, using the prevalence and total population in one location, we can compute the estimated total infections $\textsc{SeroStudy}_{\mathrm{Tinf}}$ for the past 6 months (i.e., from the beginning of the pandemic since January 2020). However, this $\textsc{SeroStudy}_{\mathrm{Tinf}}$ can not be compared with the epidemiological model estimated total infection numbers directly. The reasons are (i) the antibodies may take 10 to 14 days delay to be detectable after infection~\cite{zhao2020antibody,sethuraman2020interpreting} and (ii) the 6-14 range period for specimen collection as mentioned before. To account for this, we compare the  $\textsc{SeroStudy}_{\mathrm{Tinf}}$ numbers with the $\MDLFramework$ and $\BaseInfer$ estimated total infections of 7 days prior to the first day of specimen collection period as suggested by the CDC serological studies work~\cite{havers2020seroprevalence}.
    
    \item \textbf{Symptomatic surveillance~\cite{delphisurvey,salomon2021us}:}
    This dataset consists of point estimate $\textsc{Rate}_{\mathrm{Symp}}$ and standard error of the COVID-related symptomatic rate for each county in the US starting from April 6, 2020 to date. The survey asks a series of questions on randomly sampled social media (Facebook) users to estimate the percentage of people who have a COVID-like symptoms such as the fever along with cough or shortness of breath or difficulty breathing on a given day. However, there are several caveats such as they could not cover all symptoms of COVID-19 and these symptoms can be also caused by many other conditions, due to which they are not expected to be unbiased estimates for the true symptomatic rate~\cite{delphisurvey}. Besides, as the original symptomatic surveillance data is at a county level, we sum up the numbers to compute the $\textsc{Rate}_{\mathrm{Symp}}$ and focus on trends instead of the exact numbers.
\end{enumerate}
